DCSF: Deep Convolutional Set Functions for Classification of Asynchronous Time Series

Asynchronous Time Series is a multivariate time series where all the channels are observed asynchronously-independently, making the time series extremely sparse when aligning them. We often observe this effect in applications with complex observation processes, such as health care, climate science, and astronomy, to name a few. Because of the asynchronous nature, they pose a significant challenge to deep learning architectures, which presume that the time series presented to them are regularly sampled, fully observed, and aligned with respect to time. This paper proposes a novel framework, that we call Deep Convolutional Set Functions (DCSF), which is highly scalable and memory efficient, for the asynchronous time series classification task. With the recent advancements in deep set learning architectures, we introduce a model that is invariant to the order in which time series' channels are presented to it. We explore convolutional neural networks, which are well researched for the closely related problem-classification of regularly sampled and fully observed time series, for encoding the set elements. We evaluate DCSF for AsTS classification, and online (per time point) AsTS classification. Our extensive experiments on multiple real-world and synthetic datasets verify that the suggested model performs substantially better than a range of state-of-the-art models in terms of accuracy and run time.

==> apdx.tex <==
\appendix

\begin{table*}[t]
	\centering
	\scriptsize
	
	\begin{tabular}{|l|c c|c|c c|c|c|}
		
		\hline
		\multirow{2}{*}{Model}  & \multicolumn{3}{|c|}{Physionet} & \multicolumn{3}{|c|}{MIMIC} & \multicolumn{1}{c|}{Activity}\\
		\cline{2-8}
		& \multicolumn{2}{c|}{AUROC}                  & Time & \multicolumn{2}{c|}{AUROC} & 
		{Time} & Accuracy \\
		\hline
		GRU-D                                      & 83.2$\pm$0.3  & (81.8$\pm$0.8)       & 24s                      & \textit{85.6$\pm$0.2} & (85.7$\pm$0.2)     & 430s             & (86.2$\pm$0.5)        \\
		GRU-Simple                                 & 76.0$\pm$0.5   &       & 43s                      & 82.7$\pm$0.1    & (82.8$\pm$0.0)         & 424s                    &  \\
		IP-NETS                                    & \textit{84.2$\pm$0.4} & (81.9$\pm$0.6)& 6s                       & 84.2$\pm$0.2    &(83.2$\pm$0.5)          & 297s        & (86.9$\pm$0.7)      \\
		Phased-LSTM                                & 75.5$\pm$1.0 & (83.6$\pm$0.6)        & 46s                      & 78.9$\pm$0.3    &   (80.3$\pm$0.4)       & 452s                    & (85.5$\pm$0.5) \\
		Latent-ODE                                 &        & (82.9$\pm$0.4)              &                          &                &  (80.9$\pm$0.2)         &           &             (87.0$\pm$2.8)  \\
		SEFT-ATTN                                  & 81.8$\pm$0.4 &     (79.5$\pm$1.5)    & 4s                       & 85.0$\pm$0.2  &   (83.9$\pm$0.4)         & 29s                  &	(81.5$\pm$0.2)    \\
		mTAN                                      & 83.3$\pm$0.1 & (85.8$\pm$0.4)         &                     {\underline{3s}}     & 84.0$\pm$0.4         &     &     9s                & (\textit{91.0$\pm$0.2})     \\
		\hline
		%		ResNET-mean                                &                       &                          &                           &                          \\
		ResNET                                     & 77.8$\pm$0.7 &         & 6s                       & 81.5$\pm$0.6            &   &         &                 \\
		ResNET-mean&78.7$\pm$0.8& &18s&&&&\\
		ResNET-forward&77.4$\pm$2.2& &19s&&&&\\
		\hline
		Prop-Model w$\setminus$o time                              & \textbf{85.9$\pm$0.4}& & 10s                      & \textbf{85.6$\pm$0.1}  &   & 25s             & \textbf{91.5$\pm$0.1}         \\ %prop w/o t
				Prop-Model                                 & {84.3$\pm$0.4} &                        &            {84.6$\pm$0.1}   &                        \\
		\hline
	\end{tabular}
	\caption{Comparison of the results over two medical datasets namely Physionet2012 and Mortality (MIMIC). Best results are presented in bold and the second best are presented in italics. Time per epoch for mTAN model is lower than the presented one.}
%	\label{tab:med_data_results}
\end{table*}

\begin{table*}[ht]
	\centering
	\scriptsize
	\begin{tabular}{|l|c|c|c|c|c|c|}
		\hline
		
		& \multicolumn{3}{c|}{Phoneme Spectra} & \multicolumn{3}{c|}{LSST}\\
		\hline
		& 10\%              & 50\% & 90\% & 10\%                  & 50\% & 90\% \\
		\hline
		GRU-D                              &        & 15.8$\pm$0.6          &           &            & 51.2$\pm$0.5              &                       \\
		GRU-Simple                          &       & 11.1$\pm$0.2          &                       && 55.7$\pm$0.8              &                       \\
		IP-NETS                              &      & 16.7$\pm$0.6          &                      & 65.4$\pm$0.4 & {59.0$\pm$0.3}     & 41.0$\pm$1.2                      \\
		Phased-LSTM                           &     & 06.2$\pm$0.3          &  & & 48.8$\pm$1.1              &    40.3$\pm$0.7\\
		Latent-ODE                             &    &                       &                          & &                          &                          \\
		SEFT-ATTN                               &   & 10.9$\pm$0.7          &		&60.0$\pm$2.1	&	47.3$\pm$1.3	&	46.7$\pm$0.7	\\
		mTAN                                     &  & 11.8$\pm$0.5          &                   && 39.1$\pm$0.4              &                     \\
		\hline
		%ResNET-mean                                &                       &                          &                           &                          \\
		ResNET                                 &    & 12.7$\pm$0.6          &                          && {58.7$\pm$2.2}     &                          \\
		ResNET-mean &	24.7$\pm$0.5	&	17.9$\pm$0.6	&	11.7$\pm$0.7	&	61.3$\pm$1.1	&56.5$\pm$1.8	&	42.0$\pm$1.3\\
		ResNET-forward	&	29.0$\pm0.7$	&	19.5$\pm$0.7	&	11.4$\pm$0.2	&	64.5$\pm$2.2	&	59.1$\pm$1.3	&	44.7$\pm$0.4\\
		\hline
		Prop-Model w$\setminus$o time	& 26.8$\pm$0.6	&	\textbf{23.2$\pm$0.4}	& 13.3$\pm$0.3	&	64.9$\pm$0.3	&	\textbf{60.0$\pm$1.0}	&	44.9$\pm$1.1\\  % w$\setminus$o time 
		Prop-Model                      &           & \textit{19.9$\pm$0.9} &                       & & \textbf{60.2$\pm$0.6}              & 2s                       \\
		\hline
		Default Rate                     &          \multicolumn{3}{c|}{2.6}&\multicolumn{3}{c|}{31.5} \\
		Clas. full data & \multicolumn{3}{c|}{31.8} & \multicolumn{3}{c|}{70.19}\\
		\hline
	\end{tabular}
	\caption{Comparison of the results over two synthetic datasets namely Phoneme Spectra and LSST. Artificially induced $10\%, 50\%, 90\%$ sparsity to the dataset by randomly removing the observations. Best results are presented in bold and the second best are presented in italics.}
\end{table*}

\begin{table}[ht]
	\centering
	\scriptsize
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		
		& \multicolumn{2}{l|}{Phoneme Spectra} & \multicolumn{2}{c|}{LSST}\\
		\hline
		& Accuracy              & {Time} & Accuracy                  & {Time} \\
		\hline
		GRU-D                                      & 08.3$\pm$0.5          & 69s                      & 39.0$\pm$0.5              & 19s                      \\
		GRU-Simple                                 &     07.4$\pm$0.7      & 20s                      &      37.0$\pm$0.8         & 10s                      \\
		IP-NETS                                    & 08.6$\pm$0.4          & 292s                     & 38.3$\pm$0.3     & 21s                      \\
		Phased-LSTM                                &           & 47s                      &      37.8$\pm$0.4         & 19s                      \\
		Latent-ODE                                 &                       &                          &                           &                          \\
		SEFT-ATTN                                  & 09.2$\pm$0.5          & 4s                       & 39.1$\pm$1.1              & 3s                       \\
		mTAN                                       &     08.7$\pm$0.2      &        7s                  &       36.5$\pm$1.3        &                     \underline{1s}     \\
		\hline
		%		ResNET-mean                                &                       &                          &                           &                          \\
		ResNET                                     &           &                          &      &                          \\
		ResNET-mean &	9.2$\pm$1.0	&&39.0$\pm$1.1&\\
		ResNET-forward &	11.8$\pm$0.5	&&38.3$\pm$1.1&\\
		\hline
		Prop-Model  w$\setminus$o time                             & \textbf{11.0$\pm$0.2} & 2s                       &     \textbf{40.5$\pm$0.6}          & 2s                       \\    
				Prop-Model                                 & \textit{10.7$\pm$0.5} & 2s                       &    \textit{40.2$\pm$0.6}           & 2s                       \\
		\hline
		Default Rate                               & 2.6                   &                          & 31.5                      &                         \\
		%		Best & 31.8 & & 70.19 & \\
		\hline
	\end{tabular}
	\caption{Comparison of the results over two synthetic datasets namely Phoneme Spectra and LSST. Sampled the channels at different rates. Best results are presented in bold and the second best are presented in italics.}
\end{table}


\begin{table}[ht]
	\centering
	\scriptsize
	\begin{tabular}{|l|ccc|}
		\hline
		 \multirow{2}{*}{Dataset Aggregation type} & \multicolumn{3}{c|}{Aggregation type} \\
		\cline{2-4}
		& Sum & Average & W. Agerage \\
%		& Physionet & MIMIC \\
		\hline
		Physionet	&	86.2$\pm$0.3	&	85.9$\pm$0.4	&	\textbf{86.4$\pm$0.5} \\
		\hline
		MIMIC	&	\textbf{85.9$\pm$0.1}	&	85.6$\pm$0.1	&	85.7$\pm$0.5\\
		\hline
		Activity	&	\textbf{91.5$\pm$0.1}	&	\textbf{91.5$\pm$0.1}	&	91.3$\pm$0.1\\
		\hline
		LSST (p = 10)	&	\textbf{67.6$\pm$0.6}	&	64.9$\pm$0.3	&	66.6$\pm$0.8\\
		\hline
		LSST (p = 50)	&	58.4$\pm$1.3	&	\textbf{60.0$\pm$1.0}	&	58.3$\pm$0.6\\
		\hline
		LSST (p = 90)	&	\textbf{45.4$\pm$0.4}	&	44.9$\pm$1.1	&	45.1$\pm$0.3\\
		\hline
		LSST (VSF)	&	39.4$\pm$1.0	&	\textbf{40.5$\pm$0.6}	&	40.3$\pm$0.4\\
		\hline
		PhonemeSpectra (p = 10)	&	\textbf{29.7$\pm$0.8}	&	26.8$\pm$0.6	&	24.8$\pm$1.2	\\
		\hline
		PhonemeSpectra (p = 50)	&	23.0$\pm$0.8	&	\textbf{23.2$\pm$0.4}	&	21.7$\pm$0.3\\
		\hline
		PhonemeSpectra (p = 90)	&	13.1$\pm$0.3	&	\textbf{13.3$\pm$0.3}	&	11.8$\pm$0.7\\
		\hline
		PhonemeSpectra (VSF)	&	10.3$\pm$0.3	&	\textbf{11.0$\pm$0.2}	&	9.7$\pm$0.3\\
		\hline
	\end{tabular}
\end{table}


==> limits.tex <==
\section{Limitations}
\label{sec:limit}

Though the proposed model is simple, and provide state-of-the-art results for AsTSC (experimental results are presented in Section~\ref{sec:exps}), it has the following limitations:

\subsection{Importance of time information}

For many AsTS datasets, relative position of signals is more useful compared to their absolute locations (which are useful for forecasting problems). In fact, we could not find any AsTS dataset where absolute time information is necessary for performing the classification task. We observed that, when there is no correlation between channel interactions over time and the class label, using time information in the input is reducing the performance of the model because of the inherent bias present in the model~\cite{LK21}. A classification model always looks for the shortcut in order to classify the dataset, and if the relative positions which can be obtained from the sequence of values are sufficient for the task, time information is considered being redundant. Hence, we did not use time information while inputting the data to the encoder, meaning our input to the encoder contains only channel indicator and values, which is of dimension $\R^{{P+1}\times *}$. We empirically found that time information is necessary when there are strong correlations among the channels towards the classification label (see Section~\ref{sec:toyexp}).

%, absolute time information may not be useful in all the cases. However, relative positions of the signals carry more importance for classification.
% Though using time information is useful in the dataset containing strong temporal dependencies over time which is observed mostly for time series forecasting, using absolute time information in time series classification may not he useful, in fact it reduces the performance, because requires relative location rather than the absolute time of signals. Another reason is the inherent bias present in the model. Model tends to look at the easy places where one could find the signal for classification\cite{LK21}.

%We observed that providing time information in fact reduces the performance of the proposed model. 

\subsection{Challenges with batching during training}

Though the proposed model is extremely fast and highly scalable in theory, because we consider only the observed values, the runtime and memory depend on the platform of coding. Unfortunately, neither Tensorflow nor Pytorch support masking for the convolutional neural networks. It has a problem during batching the data while training. Because length of channels vary across the time series and data, we need to pad zeros at the end of the series in order to make a batch of data points consistent, which increases run time and memory slightly. Of course, we multiply them with zeros after convolution so that gradients will not be passed through the zero padding.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

%\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

